Accountable Fine-grained Blockchain Rewriting in the Permissionless Setting

Blockchain rewriting with fine-grained access control allows a user to create a transaction associated with a set of attributes, while another user (or modifier) who possesses enough rewriting privileges from a trusted authority satisfying the attribute set can rewrite the transaction. However, it lacks accountability and is not designed for open blockchains that require no trust assumptions. In this work, we introduce accountable fine-grained blockchain rewriting in a permissionless setting. The property of accountability allows the modifier's identity and her rewriting privileges to be held accountable for the modified transactions in case of malicious rewriting (e.g., modify the registered content from good to bad). We first present a generic framework to secure blockchain rewriting in the permissionless setting. Second, we present an instantiation of our approach and show its practicality through evaluation analysis. Last, we demonstrate that our proof-of-concept implementation can be effectively integrated into open blockchains.

==> abe.tex <==
We fully implement our proposed instantiation using Charm framework v0.43 and evaluate its 
performance on a PC with Intel Core i5 (2.7GHz $\times$ 2) and 8GB RAM.
In particular, we use GMP v6.2.0, Pairing-Based Cryptography (PBC) Library v0.5.14 
and MNT224 curve for pairing, which is the best Type-III paring in PBC.
We instantiate the hash function and the pseudo-random generator with the corresponding standard interfaces provided by the Charm framework. 
To investigate its feasibility and confirm the stated properties,
we further implemented a Proof-of-Work blockchain with interactive client in Python v3.6.7
and Flask framework v1.1.1.
The implementation code is available on GitHub (bowen: to update link).

The \texttt{Setup} algorithm takes about 0.58 seconds (s). 
The running time of \texttt{KeyGen}, \texttt{Hash}, and \texttt{Adapt} algorithms are measured and shown in \autoref{fig:runtime}. 
The performance of these algorithms is linear to the number of attributes or the size of polices. 
Specifically, the run-time of \texttt{KeyGen} is 1.99 seconds, even if the size of policies is 100.
It only takes 1.90 and 3.87 seconds respectively for \texttt{Hash} and \texttt{Adapt}
to handle a list with 100 attributes.

\begin{figure*}[bt!]
  \centering
\begin{subfigure}{.3\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Size of Policies},
    ylabel={Runtime (s)},
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.23) (20,0.44) (30,0.67) (40,0.87) (50, 1.07) (60, 1.28) (70, 1.47) (80, 1.65) (90, 1.80) (100, 1.99)
};
    % \legend{Super,Method,Argument,Arg. (one-time)}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-keygen}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    % xtick={0,1,...,4},
    % xtick={1,2,3,4},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.31) (20,0.53) (30,0.73) (40,0.92) (50, 1.13) (60, 1.28) (70, 1.46) (80, 1.63) (90, 1.75) (100, 1.90)
};
    % \legend{}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-hash}
\end{subfigure}
\begin{subfigure}{.30\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.8,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.57) (20,0.95) (30,1.33) (40,1.81) (50, 2.13) (60, 2.47) (70, 2.80) (80, 3.19) (90, 3.52) (100, 3.87)
};
    % \legend{}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-adapt}
\end{subfigure}
\caption{Running time of KeyGen (left), Hash (middle) and Adapt (right) algorithms.}
\label{fig:runtime}
\end{figure*}








We further evaluate the running time cost for proposed DPSS protocol with different
(t, n) pair, where $n$ indicates the number of committees and 
$t$ is the threshold.
The full DPSS protocol is involved in two steps, i.e., reshare and update,
and the overhead is the distribution cost between committee members, in addition to
the polynomial calculation cost.
As depicted in \autoref{fig:runtime-dpss},
the overall running time is increasing with the size of committee group scales,
since more shares would be distributed.
We further give an insight on particular timing in \autoref{table:dpss}.
The time cost is only 0.019 seconds for a 5-committee group.
With the size of group is increasing, we show that the overall cost is still low.
Therefore, we could conclude that our designed DPSS protocol is practical and cost-friendly.



\begin{table*}[!t]
 \caption{The running time cost for different (threshold, committee) pair.}
 \label{table:dpss}
 \centering
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Cost} & \multicolumn{9}{c}{(threshold, committee)} \\ \cmidrule{2-10}
                  & (2,5)   & (3,7)   & (4,9) & (5,11) & (6,13) &(7,15) &(8,17) &(9,19) &(10,21)\\ \midrule
Runtime (s)       & 0.019     & 0.036    & 0.062 & 0.123 & 0.210 &0.292 &0.386 & 0.482 &0.681\\\bottomrule
\end{tabular}
\end{table*}


\begin{figure}[bt!]
  \centering
\begin{tikzpicture}[scale = 0.8,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={2,3,4,5,6,7,8,9,10},
    symbolic x coords={2,3,4,5,6,7,8,9,10},
    ytick distance=0.2,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Size of threshold},
    ylabel={Runtime (s)},
]
\addplot [mark options={blue}, mark=square*, mark size=4pt, style={blue}] coordinates {
    (2,0.019) (3,0.036) (4,0.062) (5, 0.123) (6, 0.210) (7, 0.292) (8, 0.386) (9, 0.482) (10, 0.681)
};
\end{axis}
\end{tikzpicture}
\caption{Running time of DPSS protocol.}
\label{fig:runtime-dpss}
\end{figure}

==> new version/abe.tex <==
We fully implement our proposed instantiation using Charm framework v0.43 and evaluate its 
performance on a PC with Intel Core i5 (2.7GHz $\times$ 2) and 8GB RAM.
In particular, we use GMP v6.2.0, Pairing-Based Cryptography (PBC) Library v0.5.14 
and MNT224 curve for pairing, which is the best Type-III paring in PBC.
We instantiate the hash function and the pseudo-random generator with the corresponding standard interfaces provided by the Charm framework. 
To investigate its feasibility and confirm the stated properties,
we further implemented a Proof-of-Work blockchain with interactive client in Python v3.6.7
and Flask framework v1.1.1.
The implementation code is available on GitHub (bowen: to update link).

The \texttt{Setup} algorithm takes about 0.58 seconds (s). 
The running time of \texttt{KeyGen}, \texttt{Hash}, and \texttt{Adapt} algorithms are measured and shown in \autoref{fig:runtime}. 
The performance of these algorithms is linear to the number of attributes or the size of polices. 
Specifically, the run-time of \texttt{KeyGen} is 1.99 seconds, even if the size of policies is 100.
It only takes 1.90 and 3.87 seconds respectively for \texttt{Hash} and \texttt{Adapt}
to handle a list with 100 attributes.

\begin{figure*}[bt!]
  \centering
\begin{subfigure}{.3\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Size of Policies},
    ylabel={Runtime (s)},
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.23) (20,0.44) (30,0.67) (40,0.87) (50, 1.07) (60, 1.28) (70, 1.47) (80, 1.65) (90, 1.80) (100, 1.99)
};
    % \legend{Super,Method,Argument,Arg. (one-time)}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-keygen}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    % xtick={0,1,...,4},
    % xtick={1,2,3,4},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.31) (20,0.53) (30,0.73) (40,0.92) (50, 1.13) (60, 1.28) (70, 1.46) (80, 1.63) (90, 1.75) (100, 1.90)
};
    % \legend{}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-hash}
\end{subfigure}
\begin{subfigure}{.30\textwidth}
  \centering
\begin{tikzpicture}[scale = 0.6,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick distance=0.8,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.57) (20,0.95) (30,1.33) (40,1.81) (50, 2.13) (60, 2.47) (70, 2.80) (80, 3.19) (90, 3.52) (100, 3.87)
};
    % \legend{}
\end{axis}
\end{tikzpicture}
  \label{fig:runtime-adapt}
\end{subfigure}
\caption{Running time of KeyGen (left), Hash (middle) and Adapt (right) algorithms.}
\label{fig:runtime}
\end{figure*}








We further evaluate the running time cost for proposed DPSS protocol with different
(t, n) pair, where $n$ indicates the number of committees and 
$t$ is the threshold.
The full DPSS protocol is involved in two steps, i.e., reshare and update,
and the overhead is the distribution cost between committee members, in addition to
the polynomial calculation cost.
As depicted in \autoref{fig:runtime-dpss},
the overall running time is increasing with the size of committee group scales,
since more shares would be distributed.
We further give an insight on particular timing in \autoref{table:dpss}.
The time cost is only 0.019 seconds for a 5-committee group.
With the size of group is increasing, we show that the overall cost is still low.
Therefore, we could conclude that our designed DPSS protocol is practical and cost-friendly.



\begin{table*}[!t]
 \caption{The running time cost for different (threshold, committee) pair.}
 \label{table:dpss}
 \centering
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{Cost} & \multicolumn{9}{c}{(threshold, committee)} \\ \cmidrule{2-10}
                  & (2,5)   & (3,7)   & (4,9) & (5,11) & (6,13) &(7,15) &(8,17) &(9,19) &(10,21)\\ \midrule
Runtime (s)       & 0.019     & 0.036    & 0.062 & 0.123 & 0.210 &0.292 &0.386 & 0.482 &0.681\\\bottomrule
\end{tabular}
\end{table*}


\begin{figure}[bt!]
  \centering
\begin{tikzpicture}[scale = 0.8,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={2,3,4,5,6,7,8,9,10},
    symbolic x coords={2,3,4,5,6,7,8,9,10},
    ytick distance=0.2,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={Size of threshold},
    ylabel={Runtime (s)},
]
\addplot [mark options={blue}, mark=square*, mark size=4pt, style={blue}] coordinates {
    (2,0.019) (3,0.036) (4,0.062) (5, 0.123) (6, 0.210) (7, 0.292) (8, 0.386) (9, 0.482) (10, 0.681)
};
\end{axis}
\end{tikzpicture}
\caption{Running time of DPSS protocol.}
\label{fig:runtime-dpss}
\end{figure}

==> new version/adapt.tex <==
\begin{tikzpicture}[scale = 0.5,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %ytick distance=0.8,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={(c) Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.57) (20,0.95) (30,1.33) (40,1.81) (50, 2.13) (60, 2.47) (70, 2.80) (80, 3.19) (90, 3.52) (100, 3.87)
};
    % \legend{}
\end{axis}
\end{tikzpicture}

==> new version/dpss.tex <==
\begin{tikzpicture}[scale = 0.5,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={2,3,4,5,6,7,8,9,10},
    symbolic x coords={2,3,4,5,6,7,8,9,10},
    %ytick distance=0.2,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={(d) Size of threshold},
    ylabel={Runtime (s)},
]
\addplot [mark options={blue}, mark=square*, mark size=4pt, style={blue}] coordinates {
    (2,0.019) (3,0.036) (4,0.062) (5, 0.123) (6, 0.210) (7, 0.292) (8, 0.386) (9, 0.482) (10, 0.681)
};
\end{axis}
\end{tikzpicture}

==> new version/hash.tex <==
\begin{tikzpicture}[scale = 0.5,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    % xtick={0,1,...,4},
    % xtick={1,2,3,4},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={(b) Number of Attributes},
    ylabel={Runtime (s)}
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.38) (20,0.69) (30,0.97) (40,1.18) (50, 1.36) (60, 1.54) (70, 1.74) (80, 1.92) (90, 2.15) (100, 2.40)
};
    % \legend{}
\end{axis}
\end{tikzpicture}

==> new version/keygen.tex <==
\begin{tikzpicture}[scale = 0.5,>=stealth]
\begin{axis}[
    legend cell align={left},
    xtick={10, 20,...,100},
    symbolic x coords={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %ytick distance=0.4,
    % grid=major,
    yticklabel style={
            /pgf/number format/.cd,
            fixed,
            fixed zerofill,
            precision=1,
        	/tikz/.cd
    },
    legend style={
    at={(0,0)},
    anchor=north west,at={(axis description cs:0,1.0)}},
    xlabel={(a) Size of Policies},
    ylabel={Runtime (s)},
]
\addplot [mark options={red}, mark=square*, mark size=4pt, style={red}] coordinates {
    (10, 0.33) (20,0.50) (30,0.71) (40,0.91) (50, 1.15) (60, 1.34) (70, 1.58) (80, 1.81) (90, 2.10) (100, 2.37)
};
    % \legend{Super,Method,Argument,Arg. (one-time)}
\end{axis}
\end{tikzpicture}

==> new version/mydefs.tex <==
\usepackage{amsmath,amsfonts}
\usepackage[caption=false]{subfig}

\pagestyle{plain}%

\input{stdeqn}


%\newcommand{\G}{{\mathbb{G}}}

\newcommand{\sid}{{\textsf{sid}}}
\newcommand{\pid}{{\textsf{pid}}}

% one-time signature
\newcommand{\ots}{{\mathsf{OTS}}}
\newcommand{\otskg}{{\mathsf{KG}}}
\newcommand{\otssig}{{\mathsf{Sig}}}
\newcommand{\otsver}{{\mathsf{Ver}}}


\newcommand{\accept}{{\textsf{accept}}}
\newcommand{\reject}{{\textsf{reject}}}


\newcommand{\id}{{\tt ID}}
\newcommand{\olid}{{\overline{\id}}}
\newcommand{\h}{{\tt H}}
\newcommand{\e}{{\mathsf{\hat{e}}}}
\newcommand{\mpk}{{\tt mpk}}
\newcommand{\msk}{{\tt msk}}
\newcommand{\sk}{{\tt sk}}
\newcommand{\pk}{{\tt pk}}

\newcommand{\ask}{{\tt ask}}
\newcommand{\apk}{{\tt apk}}

\newcommand{\ibms}{{\textsf{IBMS}}}

\newcommand{\mkg}{{\textsf{MKeyGen}}}
\newcommand{\kg}{{\textsf{KeyGen}}}
\newcommand{\extract}{{\textsf{Extract}}}
\newcommand{\sign}{{\textsf{Sign}}}
\newcommand{\vrfy}{{\textsf{Verify}}}
\newcommand{\combine}{{\textsf{Combine}}}
\newcommand{\mvrfy}{{\textsf{MVerify}}}

\newcommand{\oext}{{O_{\textsf{ext}}}}
\newcommand{\osig}{{O_{\textsf{sig}}}}
\newcommand{\oh}{{O_{\textsf{H}}}}
\newcommand{\wosig}{{WO_{\textsf{sig}}}}


\newcommand{\abort}{{\tt abort}}

\newcommand{\pr}{{\mathrm{Pr}}}

\newcommand{\getsr}{{\gets_R}}
\newcommand{\iseq}{{\stackrel{?}{=}}}

\newcommand{\fullid}{{\mathsf{Full}\text{-}\mathsf{ID}}}
\newcommand{\weakid}{{\mathsf{Weak}\text{-}\mathsf{ID}}}
\newcommand{\selectiveid}{{\mathsf{Selective}\text{-}\mathsf{ID}}}
\newcommand{\eufcma}{{\mathsf{EUF}\text{-}\mathsf{CMA}}}

\newcommand{\adv}{{\mathtt{Adv}}}
\newcommand{\event}{{\mathsf{E}}}

\newcommand{\pmgen}{{\mathsf{PMGen}}}

\newcommand{\crs}{{\texttt{crs}}}
\newcommand{\tg}{{\mathsf{tag}}}


==> new version/stdeqn.tex <==
% Frequently-used equation definitions

\newcommand{\bdfn}{\begin{dfn}	\rm}
\newcommand{\edfn}{\end{dfn}}
\newcommand{\bthm}{\begin{thm}	\rm}
\newcommand{\ethm}{\end{thm}}
\newcommand{\blem}{\begin{lem}	\rm}
\newcommand{\elem}{\end{lem}}
\newcommand{\bcor}{\begin{cor}	\rm}
\newcommand{\ecor}{\end{cor}}
\newcommand{\bexa}{\begin{exa}	\rm}
\newcommand{\eexa}{\hfill$\Box$\end{exa}}
\newcommand{\bexr}{\begin{exr}	\rm}
\newcommand{\eexr}{\end{exr}}
\newcommand{\bpbm}{\begin{pbm}	\rm}
\newcommand{\epbm}{\end{pbm}}

\newcommand{\Z}{{\mathbb{Z}_q}}
\newcommand{\N}{{\mathbb{N}}}

\newcommand{\EQ}{\begin{eqnarray*}}
\newcommand{\EN}{\end{eqnarray*}}
\newcommand{\eq}{\begin{eqnarray}}
\newcommand{\en}{\end{eqnarray}}

\newcommand{\Sym}{{\mathrm{Sym}}}
\newcommand{\prob}{{\mathrm{Pr}}}

\newcommand{\sinc}{\mbox{\rm sinc}}
\newcommand{\bfitnu}{\mbox{\boldmath $nu$}}
\newcommand{\bfitc}{\mbox{\boldmath $c$}}
\newcommand{\bfitr}{\mbox{\boldmath $r$}}
\newcommand{\erfc}{\mbox{\rm erfc}}
\newcommand{\define}{{\stackrel{\triangle}{\to}}}
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\lcm}{{\mathrm{lcm}}}

\newcommand{\bfzero}{\mbox{\bf 0}}

\newcommand{\asup}[1]{\mbox{$\alpha^{#1}$}}
\newcommand{\bsup}[1]{\mbox{$\beta^{#1}$}}

\newcommand{\checka}{{\check{a}}}
\newcommand{\checkb}{{\check{b}}}
\newcommand{\checkc}{{\check{c}}}
\newcommand{\checkd}{{\check{d}}}
\newcommand{\checke}{{\check{e}}}
\newcommand{\checkf}{{\check{f}}}
\newcommand{\checkg}{{\check{g}}}
\newcommand{\checkh}{{\check{h}}}
\newcommand{\checki}{{\check{i}}}
\newcommand{\checkj}{{\check{j}}}
\newcommand{\checkk}{{\check{k}}}
\newcommand{\checkl}{{\check{l}}}
\newcommand{\checkm}{{\check{m}}}
\newcommand{\checkn}{{\check{n}}}
\newcommand{\checko}{{\check{o}}}
\newcommand{\checkp}{{\check{p}}}
\newcommand{\checkq}{{\check{q}}}
\newcommand{\checkr}{{\check{r}}}
\newcommand{\checks}{{\check{s}}}
\newcommand{\checkt}{{\check{t}}}
\newcommand{\checku}{{\check{u}}}
\newcommand{\checkv}{{\check{v}}}
\newcommand{\checkw}{{\check{w}}}
\newcommand{\checkx}{{\check{x}}}
\newcommand{\checky}{{\check{y}}}
\newcommand{\checkz}{{\check{z}}}

\newcommand{\checkA}{{\check{A}}}
\newcommand{\checkB}{{\check{B}}}
\newcommand{\checkC}{{\check{C}}}
\newcommand{\checkD}{{\check{D}}}
\newcommand{\checkE}{{\check{E}}}
\newcommand{\checkF}{{\check{F}}}
\newcommand{\checkG}{{\check{G}}}
\newcommand{\checkH}{{\check{H}}}
\newcommand{\checkI}{{\check{I}}}
\newcommand{\checkJ}{{\check{J}}}
\newcommand{\checkK}{{\check{K}}}
\newcommand{\checkL}{{\check{L}}}
\newcommand{\checkM}{{\check{M}}}
\newcommand{\checkN}{{\check{N}}}
\newcommand{\checkO}{{\check{O}}}
\newcommand{\checkP}{{\check{P}}}
\newcommand{\checkQ}{{\check{Q}}}
\newcommand{\checkR}{{\check{R}}}
\newcommand{\checkS}{{\check{S}}}
\newcommand{\checkT}{{\check{T}}}
\newcommand{\checkU}{{\check{U}}}
\newcommand{\checkV}{{\check{V}}}
\newcommand{\checkW}{{\check{W}}}
\newcommand{\checkX}{{\check{X}}}
\newcommand{\checkY}{{\check{Y}}}
\newcommand{\checkZ}{{\check{Z}}}

\newcommand{\hata}{{\hat{a}}}
\newcommand{\hatb}{{\hat{b}}}
\newcommand{\hatc}{{\hat{c}}}
\newcommand{\hatd}{{\hat{d}}}
\newcommand{\hate}{{\hat{e}}}
\newcommand{\hatf}{{\hat{f}}}
\newcommand{\hatg}{{\hat{g}}}
\newcommand{\hath}{{\hat{h}}}
\newcommand{\hati}{{\hat{i}}}
\newcommand{\hatj}{{\hat{j}}}
\newcommand{\hatk}{{\hat{k}}}
\newcommand{\hatl}{{\hat{l}}}
\newcommand{\hatm}{{\hat{m}}}
\newcommand{\hatn}{{\hat{n}}}
\newcommand{\hato}{{\hat{o}}}
\newcommand{\hatp}{{\hat{p}}}
\newcommand{\hatq}{{\hat{q}}}
\newcommand{\hatr}{{\hat{r}}}
\newcommand{\hats}{{\hat{s}}}
\newcommand{\hatt}{{\hat{t}}}
\newcommand{\hatu}{{\hat{u}}}
\newcommand{\hatv}{{\hat{v}}}
\newcommand{\hatw}{{\hat{w}}}
\newcommand{\hatx}{{\hat{x}}}
\newcommand{\haty}{{\hat{y}}}
\newcommand{\hatz}{{\hat{z}}}

\newcommand{\hatA}{{\hat{A}}}
\newcommand{\hatB}{{\hat{B}}}
\newcommand{\hatC}{{\hat{C}}}
\newcommand{\hatD}{{\hat{D}}}
\newcommand{\hatE}{{\hat{E}}}
\newcommand{\hatF}{{\hat{F}}}
\newcommand{\hatG}{{\hat{G}}}
\newcommand{\hatH}{{\hat{H}}}
\newcommand{\hatI}{{\hat{I}}}
\newcommand{\hatJ}{{\hat{J}}}
\newcommand{\hatK}{{\hat{K}}}
\newcommand{\hatL}{{\hat{L}}}
\newcommand{\hatM}{{\hat{M}}}
\newcommand{\hatN}{{\hat{N}}}
\newcommand{\hatO}{{\hat{O}}}
\newcommand{\hatP}{{\hat{P}}}
\newcommand{\hatQ}{{\hat{Q}}}
\newcommand{\hatR}{{\hat{R}}}
\newcommand{\hatS}{{\hat{S}}}
\newcommand{\hatT}{{\hat{T}}}
\newcommand{\hatU}{{\hat{U}}}
\newcommand{\hatV}{{\hat{V}}}
\newcommand{\hatW}{{\hat{W}}}
\newcommand{\hatX}{{\hat{X}}}
\newcommand{\hatY}{{\hat{Y}}}
\newcommand{\hatZ}{{\hat{Z}}}

\newcommand{\overlinea}{{\overline{a}}}
\newcommand{\overlineb}{{\overline{b}}}
\newcommand{\overlinec}{{\overline{c}}}
\newcommand{\overlined}{{\overline{d}}}
\newcommand{\overlinee}{{\overline{e}}}
\newcommand{\overlinef}{{\overline{f}}}
\newcommand{\overlineg}{{\overline{g}}}
\newcommand{\overlineh}{{\overline{h}}}
\newcommand{\overlinei}{{\overline{i}}}
\newcommand{\overlinej}{{\overline{j}}}
\newcommand{\overlinek}{{\overline{k}}}
\newcommand{\overlinel}{{\overline{l}}}
\newcommand{\overlinem}{{\overline{m}}}
\newcommand{\overlinen}{{\overline{n}}}
\newcommand{\overlineo}{{\overline{o}}}
\newcommand{\overlinep}{{\overline{p}}}
\newcommand{\overlineq}{{\overline{q}}}
\newcommand{\overliner}{{\overline{r}}}
\newcommand{\overlines}{{\overline{s}}}
\newcommand{\overlinet}{{\overline{t}}}
\newcommand{\overlineu}{{\overline{u}}}
\newcommand{\overlinev}{{\overline{v}}}
\newcommand{\overlinew}{{\overline{w}}}
\newcommand{\overlinex}{{\overline{x}}}
\newcommand{\overliney}{{\overline{y}}}
\newcommand{\overlinez}{{\overline{z}}}

\newcommand{\overlineA}{{\overline{A}}}
\newcommand{\overlineB}{{\overline{B}}}
\newcommand{\overlineC}{{\overline{C}}}
\newcommand{\overlineD}{{\overline{D}}}
\newcommand{\overlineE}{{\overline{E}}}
\newcommand{\overlineF}{{\overline{F}}}
\newcommand{\overlineG}{{\overline{G}}}
\newcommand{\overlineH}{{\overline{H}}}
\newcommand{\overlineI}{{\overline{I}}}
\newcommand{\overlineJ}{{\overline{J}}}
\newcommand{\overlineK}{{\overline{K}}}
\newcommand{\overlineL}{{\overline{L}}}
\newcommand{\overlineM}{{\overline{M}}}
\newcommand{\overlineN}{{\overline{N}}}
\newcommand{\overlineO}{{\overline{O}}}
\newcommand{\overlineP}{{\overline{P}}}
\newcommand{\overlineQ}{{\overline{Q}}}
\newcommand{\overlineR}{{\overline{R}}}
\newcommand{\overlineS}{{\overline{S}}}
\newcommand{\overlineT}{{\overline{T}}}
\newcommand{\overlineU}{{\overline{U}}}
\newcommand{\overlineV}{{\overline{V}}}
\newcommand{\overlineW}{{\overline{W}}}
\newcommand{\overlineX}{{\overline{X}}}
\newcommand{\overlineY}{{\overline{Y}}}
\newcommand{\overlineZ}{{\overline{Z}}}


\newcommand{\bara}{{\bar{a}}}
\newcommand{\barb}{{\bar{b}}}
\newcommand{\barc}{{\bar{c}}}
\newcommand{\bard}{{\bar{d}}}
\newcommand{\bare}{{\bar{e}}}
\newcommand{\barf}{{\bar{f}}}
\newcommand{\barg}{{\bar{g}}}
\newcommand{\barh}{{\bar{h}}}
\newcommand{\bari}{{\bar{i}}}
\newcommand{\barj}{{\bar{j}}}
\newcommand{\bark}{{\bar{k}}}
\newcommand{\barl}{{\bar{l}}}
\newcommand{\barm}{{\bar{m}}}
\newcommand{\barn}{{\bar{n}}}
\newcommand{\baro}{{\bar{o}}}
\newcommand{\barp}{{\bar{p}}}
\newcommand{\barq}{{\bar{q}}}
\newcommand{\barr}{{\bar{r}}}
\newcommand{\bars}{{\bar{s}}}
\newcommand{\bart}{{\bar{t}}}
\newcommand{\baru}{{\bar{u}}}
\newcommand{\barv}{{\bar{v}}}
\newcommand{\barw}{{\bar{w}}}
\newcommand{\barx}{{\bar{x}}}
\newcommand{\bary}{{\bar{y}}}
\newcommand{\barz}{{\bar{z}}}

\newcommand{\barA}{{\bar{A}}}
\newcommand{\barB}{{\bar{B}}}
\newcommand{\barC}{{\bar{C}}}
\newcommand{\barD}{{\bar{D}}}
\newcommand{\barE}{{\bar{E}}}
\newcommand{\barF}{{\bar{F}}}
\newcommand{\barG}{{\bar{G}}}
\newcommand{\barH}{{\bar{H}}}
\newcommand{\barI}{{\bar{I}}}
\newcommand{\barJ}{{\bar{J}}}
\newcommand{\barK}{{\bar{K}}}
\newcommand{\barL}{{\bar{L}}}
\newcommand{\barM}{{\bar{M}}}
\newcommand{\barN}{{\bar{N}}}
\newcommand{\barO}{{\bar{O}}}
\newcommand{\barP}{{\bar{P}}}
\newcommand{\barQ}{{\bar{Q}}}
\newcommand{\barR}{{\bar{R}}}
\newcommand{\barS}{{\bar{S}}}
\newcommand{\barT}{{\bar{T}}}
\newcommand{\barU}{{\bar{U}}}
\newcommand{\barV}{{\bar{V}}}
\newcommand{\barW}{{\bar{W}}}
\newcommand{\barX}{{\bar{X}}}
\newcommand{\barY}{{\bar{Y}}}
\newcommand{\barZ}{{\bar{Z}}}


\newcommand{\tildea}{{\tilde{a}}}
\newcommand{\tildeb}{{\tilde{b}}}
\newcommand{\tildec}{{\tilde{c}}}
\newcommand{\tilded}{{\tilde{d}}}
\newcommand{\tildee}{{\tilde{e}}}
\newcommand{\tildef}{{\tilde{f}}}
\newcommand{\tildeg}{{\tilde{g}}}
\newcommand{\tildeh}{{\tilde{h}}}
\newcommand{\tildei}{{\tilde{i}}}
\newcommand{\tildej}{{\tilde{j}}}
\newcommand{\tildek}{{\tilde{k}}}
\newcommand{\tildel}{{\tilde{l}}}
\newcommand{\tildem}{{\tilde{m}}}
\newcommand{\tilden}{{\tilde{n}}}
\newcommand{\tildeo}{{\tilde{o}}}
\newcommand{\tildep}{{\tilde{p}}}
\newcommand{\tildeq}{{\tilde{q}}}
\newcommand{\tilder}{{\tilde{r}}}
\newcommand{\tildes}{{\tilde{s}}}
\newcommand{\tildet}{{\tilde{t}}}
\newcommand{\tildeu}{{\tilde{u}}}
\newcommand{\tildev}{{\tilde{v}}}
\newcommand{\tildew}{{\tilde{w}}}
\newcommand{\tildex}{{\tilde{x}}}
\newcommand{\tildey}{{\tilde{y}}}
\newcommand{\tildez}{{\tilde{z}}}

\newcommand{\tildeA}{{\tilde{A}}}
\newcommand{\tildeB}{{\tilde{B}}}
\newcommand{\tildeC}{{\tilde{C}}}
\newcommand{\tildeD}{{\tilde{D}}}
\newcommand{\tildeE}{{\tilde{E}}}
\newcommand{\tildeF}{{\tilde{F}}}
\newcommand{\tildeG}{{\tilde{G}}}
\newcommand{\tildeH}{{\tilde{H}}}
\newcommand{\tildeI}{{\tilde{I}}}
\newcommand{\tildeJ}{{\tilde{J}}}
\newcommand{\tildeK}{{\tilde{K}}}
\newcommand{\tildeL}{{\tilde{L}}}
\newcommand{\tildeM}{{\tilde{M}}}
\newcommand{\tildeN}{{\tilde{N}}}
\newcommand{\tildeO}{{\tilde{O}}}
\newcommand{\tildeP}{{\tilde{P}}}
\newcommand{\tildeQ}{{\tilde{Q}}}
\newcommand{\tildeR}{{\tilde{R}}}
\newcommand{\tildeS}{{\tilde{S}}}
\newcommand{\tildeT}{{\tilde{T}}}
\newcommand{\tildeU}{{\tilde{U}}}
\newcommand{\tildeV}{{\tilde{V}}}
\newcommand{\tildeW}{{\tilde{W}}}
\newcommand{\tildeX}{{\tilde{X}}}
\newcommand{\tildeY}{{\tilde{Y}}}
\newcommand{\tildeZ}{{\tilde{Z}}}

\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}

\newcommand{\bfA}{{\bf{A}}}
\newcommand{\bfB}{{\bf{B}}}
\newcommand{\bfC}{{\bf{C}}}
\newcommand{\bfD}{{\bf{D}}}
\newcommand{\bfE}{{\bf{E}}}
\newcommand{\bfF}{{\bf{F}}}
\newcommand{\bfG}{{\bf{G}}}
\newcommand{\bfH}{{\bf{H}}}
\newcommand{\bfI}{{\bf{I}}}
\newcommand{\bfJ}{{\bf{J}}}
\newcommand{\bfK}{{\bf{K}}}
\newcommand{\bfL}{{\bf{L}}}
\newcommand{\bfM}{{\bf{M}}}
\newcommand{\bfN}{{\bf{N}}}
\newcommand{\bfO}{{\bf{O}}}
\newcommand{\bfP}{{\bf{P}}}
\newcommand{\bfQ}{{\bf{Q}}}
\newcommand{\bfR}{{\bf{R}}}
\newcommand{\bfS}{{\bf{S}}}
\newcommand{\bfT}{{\bf{T}}}
\newcommand{\bfU}{{\bf{U}}}
\newcommand{\bfV}{{\bf{V}}}
\newcommand{\bfW}{{\bf{W}}}
\newcommand{\bfX}{{\bf{X}}}
\newcommand{\bfY}{{\bf{Y}}}
\newcommand{\bfZ}{{\bf{Z}}}

\newcommand{\bfa}{{\bf{a}}}
\newcommand{\bfb}{{\bf{b}}}
\newcommand{\bfc}{{\bf{c}}}
\newcommand{\bfd}{{\bf{d}}}
\newcommand{\bfe}{{\bf{e}}}
\newcommand{\bff}{{\bf{f}}}
\newcommand{\bfg}{{\bf{g}}}
\newcommand{\bfh}{{\bf{h}}}
\newcommand{\bfi}{{\bf{i}}}
\newcommand{\bfj}{{\bf{j}}}
\newcommand{\bfk}{{\bf{k}}}
\newcommand{\bfl}{{\bf{l}}}
\newcommand{\bfm}{{\bf{m}}}
\newcommand{\bfn}{{\bf{n}}}
\newcommand{\bfo}{{\bf{o}}}
\newcommand{\bfp}{{\bf{p}}}
\newcommand{\bfq}{{\bf{q}}}
\newcommand{\bfr}{{\bf{r}}}
\newcommand{\bfs}{{\bf{s}}}
\newcommand{\bft}{{\bf{t}}}
\newcommand{\bfu}{{\bf{u}}}
\newcommand{\bfv}{{\bf{v}}}
\newcommand{\bfw}{{\bf{w}}}
\newcommand{\bfx}{{\bf{x}}}
\newcommand{\bfy}{{\bf{y}}}
\newcommand{\bfz}{{\bf{z}}}


